Rising Multi-Armed Bandits with Known Horizons

Rising Multi-Armed Bandits (RMABs) model sequential decision problems where each arm's expected reward improves with repeated pulls. In such problems, the value of investing in an arm depends on how much time remains, making knowledge of the horizon useful side information, yet its benefit remains underexplored. We investigate this benefit through CURE-UCB, a horizon-aware algorithm that estimates each arm's cumulative reward over the remaining horizon. Theoretically, under structured assumptions, we prove that CURE-UCB uniformly dominates a representative horizon-agnostic algorithm and show that the advantage of horizon awareness can be substantial: on some instances, CURE-UCB incurs only $O(1)$ regret whereas the horizon-agnostic algorithm suffers $\Omega(T)$. Furthermore, we establish a regret upper bound for the general concave rising bandit setting whose growth-dependent term matches the known lower bound in its dependence on $T$. Empirically, across synthetic benchmarks and real-world model selection tasks, CURE-UCB achieves lower regret than both rising and non-stationary baselines over a wide range of horizons.

==> algorithm/R-ed-UCB.tex <==
\begin{algorithm}[!ht]
\caption{\texttt{Rested UCB\!\! (R-ed-UCB)\!\!}}\label{alg:R-ed-UCB}
	\begin{algorithmic}
	\STATE \textbf{Input} $N_{i,0} \leftarrow 0$ for all $i \in [|\gS|]$, Sliding window parameter $\varepsilon$.
	\STATE \textbf{Initialize} Play each super arm $S_{i}$ two times for each $i \in [|\gS|]$.
	\FOR{$t \in ( 1, \dots, T)$}
        \STATE Calculate Future-UCB $\Acute{\mu}_i(t)$ for each super arm.
        \STATE $S_t \leftarrow \texttt{Solver}(\acute\mu_1(t), \acute\mu_2(t), \cdots, \acute\mu_{|\gS|}(t))$.
        \STATE Play $S_t$ and observe reward $R_t$.
        \STATE Update $\gF_t$ and $N_{i,t}$.
	\ENDFOR
	\end{algorithmic}
\end{algorithm}

==> algorithm/SW-TS.tex <==
\begin{algorithm}[!ht]
\caption{\texttt{Sliding Window Thompson Sampling\!\! (SW-TS)\!\!}}\label{alg:SW-TS}
	\begin{algorithmic}
	\STATE \textbf{Input} Sliding window size $h$.
	\STATE \textbf{Initialize} Play each super arm $S_{i}$ two times for each $i \in [|\gS|]$.
	\FOR{$t \in ( 1, \dots, T)$}
        \STATE For each super arm $S_i$, set ${\theta}_i(t)\sim Beta(\alpha_{i}+1, \beta_{i}+1)$.
            \STATE $S_t \leftarrow$ $\argmax$($\theta_{1}(t), \theta_{2}(t), \cdots, \theta_{K}(t)$).
            \STATE Play $S_t$ and observe reward $X_{S_t}(t)$.
            \STATE Update $\alpha_{i}$ and $\beta_{i}$.
	\ENDFOR
	\end{algorithmic}
\end{algorithm}

==> algorithm/SW-UCB.tex <==
\begin{algorithm}[!ht]
\caption{\texttt{Sliding Window-UCB\!\! (SW-UCB)\!\!}}\label{alg:SW-UCB}
	\begin{algorithmic}
	\STATE \textbf{Input} $N_{i,0} \leftarrow 0$ for all $i \in [|\gS|]$, Sliding window size $h$.
	\STATE \textbf{Initialize} Play each super arm $S_{i}$ two times for each $i \in [|\gS|]$.
	\FOR{$t \in ( 1, \dots, T)$}
            \STATE For each super arm $S_{i}$, set $\Acute{\mu}_{i}^\texttt{SW-UCB}(t)=\hat{\mu}_{i}^\texttt{SW-UCB}(t)+\beta_{i}^\texttt{SW-UCB}(t)$.
		\STATE $S_t \leftarrow$ $\argmax$($\Acute{\mu}_{1}^\texttt{SW-UCB}(t), \Acute{\mu}_{2}^\texttt{SW-UCB}(t), \cdots, \Acute{\mu}_{|\gS|}^\texttt{SW-UCB}(t)$).
		\STATE Play $S_t$ and observe reward $X_{S_t}(t)$.
            \STATE Update $\hat{\mu}_{i}^\texttt{SW-UCB}(t)$ and $N_{i,t}$.
	\ENDFOR
	\end{algorithmic}
\end{algorithm}

==> figure/tex/IMDB_backup.tex <==
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{graphicx}

\definecolor{imdbred}{RGB}{255,0,0}
\definecolor{imdbgreen}{RGB}{0,128,0}
\definecolor{imdbblue}{RGB}{0,0,255}
\definecolor{imdbcyan}{RGB}{0,200,200}
\definecolor{imdbmagenta}{RGB}{220,0,220}
\definecolor{imdbyellow}{RGB}{180,180,0}
\definecolor{imdbgray}{RGB}{180,180,180}

\definecolor{llmgreen}{RGB}{50,160,50}
\definecolor{llmorange}{RGB}{240,140,20}
\definecolor{llmpurple}{RGB}{150,100,200}
\definecolor{llmred}{RGB}{220,40,40}
\definecolor{llmblue}{RGB}{40,120,190}

\newcommand{\legenditem}[2]{%
    \textcolor{#1}{\rule[0.6ex]{1.5em}{1.2pt}}%
    \hspace{0.35em}#2%
}

\newlength{\panelW}
\newlength{\panelH}
\newlength{\algLegendW}
\newlength{\topLegendH}

\begin{figure}[t]
    \centering

    \captionsetup{font=small}
    \captionsetup[subfigure]{
        font=footnotesize,
        labelfont=bf,
        justification=centering,
        singlelinecheck=true,
        skip=2pt
    }

    % Slightly smaller overall figure
    \setlength{\panelW}{0.455\linewidth}
    \setlength{\panelH}{0.215\textheight}
    \setlength{\algLegendW}{0.68\linewidth}
    \setlength{\topLegendH}{2.6\baselineskip}

    % =========================
    % Top row: reward dynamics
    % =========================
    \begin{subfigure}[t]{\panelW}
        \centering
        \begin{minipage}[t][\topLegendH][c]{\linewidth}
            \centering
            \scriptsize
            \legenditem{imdbred}{LR(0.003)}\hspace{0.8em}
            \legenditem{imdbgreen}{NN:(1,)}\hspace{0.8em}
            \legenditem{imdbblue}{NN:(5,)}\\[1pt]
            \legenditem{imdbcyan}{NN:(2, 2, 2)}\hspace{0.8em}
            \legenditem{imdbmagenta}{NN:(1, 1, 2)}\hspace{0.8em}
            \legenditem{imdbyellow}{NB}\hspace{0.8em}
            \legenditem{imdbgray}{OGD(0.003)}
        \end{minipage}

        \vspace{0.2ex}

        \includegraphics[
            width=0.98\linewidth,
            height=\panelH,
            keepaspectratio,
            trim={36pt 20pt 34pt 18pt},
            clip
        ]{figure/images/IMDB_reward.pdf}
        \caption{IMDB reward dynamics}
        \label{fig:imdb_reward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{\panelW}
        \centering
        \begin{minipage}[t][\topLegendH][c]{\linewidth}
            \centering
            \scriptsize
            \legenditem{llmgreen}{Qwen3.5-2B}\hspace{0.8em}
            \legenditem{llmorange}{Qwen3.5-4B}\hspace{0.8em}
            \legenditem{llmpurple}{Qwen3.5-9B}\\[1pt]
            \legenditem{llmred}{Qwen3.5-27B}\hspace{0.8em}
            \legenditem{llmblue}{Qwen3.8-Max}
        \end{minipage}

        \vspace{0.2ex}

        \includegraphics[
            width=0.98\linewidth,
            height=\panelH,
            keepaspectratio,
            trim={36pt 28pt 42pt 22pt},
            clip
        ]{figure/images/LLM_reward.pdf}
        \caption{XSum-LLM reward dynamics}
        \label{fig:llm_reward}
    \end{subfigure}

    \vspace{0.6ex}

    % =========================
    % Shared algorithm legend
    % =========================
    \includegraphics[width=\algLegendW]{figure/images/legend_all_algorithms.pdf}

    \vspace{0.6ex}

    % =========================
    % Bottom row: cumulative regret
    % =========================
    \begin{subfigure}[t]{\panelW}
        \centering
        \includegraphics[
            width=0.98\linewidth,
            height=\panelH,
            keepaspectratio,
            trim={36pt 30pt 36pt 8pt},
            clip
        ]{figure/images/regret_IMDB.pdf}
        \caption{IMDB cumulative regret}
        \label{fig:imdb_regret}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{\panelW}
        \centering
        \includegraphics[
            width=0.98\linewidth,
            height=\panelH,
            keepaspectratio,
            trim={36pt 30pt 36pt 8pt},
            clip
        ]{figure/images/LLM_regret.pdf}
        \caption{XSum-LLM cumulative regret}
        \label{fig:llm_regret}
    \end{subfigure}

    \caption{
    \textbf{Online model selection on IMDB and XSum-LLM.}
    The top row shows reward dynamics, and the bottom row shows cumulative regret.
    The left column corresponds to IMDB sentiment analysis with $T=50K$, and the right column corresponds to LLM fine-tuning on XSum summarization with $T=1K$.
    The legends above (a) and (b) indicate model configurations, and the shared legend between the two rows indicates the algorithms used in the cumulative-regret plots.
    Shaded regions denote 95\% confidence intervals over 40 seeds.
    }
    \label{fig:realworld_combined}
\end{figure}


% \newlength{\rwFigureWidth}
% \newlength{\rwPlotWidth}
% \newlength{\rwLegendWidth}

% \begin{figure}[t]
%     \centering
%     \captionsetup[subfigure]{font=small, skip=2pt}

%     % Capture the full figure width before entering any subfigure
%     \setlength{\rwFigureWidth}{\linewidth}
%     \setlength{\rwPlotWidth}{0.36\rwFigureWidth}
%     \setlength{\rwLegendWidth}{0.22\rwFigureWidth}

%     % ===== Top: shared horizontal algorithm legend =====
%     \includegraphics[width=0.82\rwFigureWidth]
%         {figure/images/legend_all_algorithms.pdf}

%     \vspace{0.4ex}

%     % ===== Top row: IMDB =====
%     \begin{subfigure}[b]{0.60\rwFigureWidth}
%         \centering
%         \begin{minipage}[c]{\rwPlotWidth}
%             \includegraphics[
%                 width=\linewidth,
%                 trim={36pt 14pt 34pt 18pt},
%                 clip
%             ]{figure/images/IMDB_reward.pdf}
%         \end{minipage}%
%         \hspace{2pt}%
%         \begin{minipage}[c]{\rwLegendWidth}
%             \raggedright
%             % Match the nominal text size of the LLM legend
%             \includegraphics[
%                 width=0.773\linewidth,
%                 trim={42pt 12pt 45pt 12pt},
%                 clip
%             ]{figure/images/legend_IMDB_model.pdf}
%         \end{minipage}
%         \caption{Reward dynamics}
%         \label{fig:imdb_reward}
%     \end{subfigure}%
%     \hspace{0.008\rwFigureWidth}%
%     \begin{subfigure}[b]{0.37\rwFigureWidth}
%         \centering
%         \includegraphics[
%             width=\rwPlotWidth,
%             trim={36pt 30pt 36pt 8pt},
%             clip
%         ]{figure/images/regret_IMDB.pdf}
%         \caption{Cumulative regret}
%         \label{fig:imdb_regret}
%     \end{subfigure}

%     \vspace{0.6ex}

%     % ===== Bottom row: LLM =====
%     \begin{subfigure}[b]{0.60\rwFigureWidth}
%         \centering
%         \begin{minipage}[c]{\rwPlotWidth}
%             \includegraphics[
%                 width=\linewidth,
%                 trim={36pt 28pt 42pt 22pt},
%                 clip
%             ]{figure/images/LLM_reward.pdf}
%         \end{minipage}%
%         \hspace{2pt}%
%         \begin{minipage}[c]{\rwLegendWidth}
%             \raggedright
%             \includegraphics[
%                 width=\linewidth,
%                 trim={14pt 50pt 16pt 52pt},
%                 clip
%             ]{figure/images/legend_LLM.pdf}
%         \end{minipage}
%         \caption{Reward dynamics}
%         \label{fig:llm_reward}
%     \end{subfigure}%
%     \hspace{0.008\rwFigureWidth}%
%     \begin{subfigure}[b]{0.37\rwFigureWidth}
%         \centering
%         \includegraphics[
%             width=\rwPlotWidth,
%             trim={36pt 30pt 36pt 8pt},
%             clip
%         ]{figure/images/LLM_regret.pdf}
%         \caption{Cumulative regret}
%         \label{fig:llm_regret}
%     \end{subfigure}

%     \caption{
%     \textbf{Online model selection on IMDB (top row) and XSum-LLM (bottom row).}
%     (a, b) IMDB sentiment analysis with $T=50K$.
%     (c, d) LLM fine-tuning on XSum summarization with $T=1K$.
%     The shared legend at the top indicates the algorithms used in the cumulative-regret plots, while the legends beside the left-column plots indicate model configurations.
%     Shaded regions denote 95\% confidence intervals over 40 seeds.
%     }
%     \label{fig:realworld_combined}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \captionsetup[subfigure]{font=small, skip=0pt}
%     \def\plotlegendgap{-0.018\linewidth}
%     % ---- size controls ----
%     \def\plotheight{0.19\textheight}
%     \def\sidelegendheight{0.1\textheight}
%     \def\plotlegendgap{-0.018\linewidth} % negative gap: pull legend closer
%     \def\rightplotheight{0.18\textheight} % b,d만 조금 더 크게
    
%     \def\fitplot#1{%
%         \includegraphics[
%             width=\linewidth,
%             height=\plotheight,
%             keepaspectratio
%         ]{#1}%
%     }

%     \def\fitplotright#1{%
%     \includegraphics[
%         width=\linewidth,
%         height=\rightplotheight,
%         keepaspectratio,
%         trim=0pt 0pt 0pt 0pt,
%         clip
%     ]{#1}%
% }
    
%     \def\fitplotleft#1{%
%         \includegraphics[
%             width=\linewidth,
%             height=\plotheight,
%             keepaspectratio,
%             trim=0pt 0pt 0pt 0pt,
%             clip
%         ]{#1}%
%     }
    
%     \def\fitmodellegend#1{%
%         \includegraphics[
%             width=\linewidth,
%             height=\sidelegendheight,
%             keepaspectratio,
%             trim=10pt 0pt 0pt 0pt,
%             clip
%         ]{#1}%
%     }
    
%     % Main block + right shared algorithm legend.
%     \def\mainblockwidth{0.825\linewidth}
%     \def\alglegendblockwidth{0.165\linewidth}
%     \def\alglegendheight{0.2\textheight}

%     \def\fitplot#1{%
%         \includegraphics[
%             width=\linewidth,
%             height=\plotheight,
%             keepaspectratio
%         ]{#1}%
%     }

%     \begin{minipage}[t]{\mainblockwidth}
%         \centering

%         % ===== Top row =====
%        \begin{subfigure}[t]{0.58\linewidth}
%         \centering
    
%         \begin{minipage}[t]{0.705\linewidth}
%             \centering
%             \begin{minipage}[c][\plotheight][c]{\linewidth}
%                 \centering
%                 \fitplotleft{figure/images/IMDB_reward_2.pdf}
%             \end{minipage}
%             \vspace{-2ex}
%             \caption{Reward dynamics}
%             \label{fig:imdb_reward}
%         \end{minipage}%
%         \hspace{\plotlegendgap}%
%         \begin{minipage}[t]{0.3\linewidth}
%             \centering
%             \begin{minipage}[c][\plotheight][c]{\linewidth}
%                 \centering
%                 \fitmodellegend{figure/images/legend_IMDB_model.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{subfigure}
%         \hfill
% \begin{subfigure}[t]{0.39\linewidth}
%     \centering
%     \begin{minipage}[c][\rightplotheight][c]{\linewidth}
%         \centering
%         \fitplotright{figure/images/IMDB_regret.pdf}
%     \end{minipage}
%     \caption{Cumulative regret}
%     \label{fig:imdb_regret}
% \end{subfigure}
%         \vspace{0.2ex}
%         % ===== Bottom row =====
%        \begin{subfigure}[t]{0.58\linewidth}
%         \centering
    
%         \begin{minipage}[t]{0.705\linewidth}
%             \centering
%             \begin{minipage}[c][\plotheight][c]{\linewidth}
%                 \centering
%                 \fitplotleft{figure/images/LLM_reward.pdf}
%             \end{minipage}
%             \vspace{-2ex}
%             \caption{Reward dynamics}
%             \label{fig:llm_reward}
%         \end{minipage}%
%         \hspace{\plotlegendgap}%
%         \begin{minipage}[t]{0.3\linewidth}
%             \centering
%             \begin{minipage}[c][\plotheight][c]{\linewidth}
%                 \centering
%                 \fitmodellegend{figure/images/legend_LLM.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{subfigure}
%         \hfill
% \begin{subfigure}[t]{0.39\linewidth}
%     \centering
%     \begin{minipage}[c][\rightplotheight][c]{\linewidth}
%         \centering
%         \fitplotright{figure/images/LLM_regret.pdf}
%     \end{minipage}

%     \caption{Cumulative regret}
%     \label{fig:llm_regret}
% \end{subfigure}
%     \end{minipage}%
%     \hspace{0.006\linewidth}%
%     % ===== Right-side shared vertical legend for (b), (d) =====
%     \begin{minipage}[t][\alglegendheight][c]{\alglegendblockwidth}
%         \centering
%         \vspace*{-0.04\textheight}
%         \includegraphics[
%             height=\alglegendheight,
%             keepaspectratio
%         ]{figure/images/legend_all_algorithms_vertical.pdf}
%     \end{minipage}

%     \caption{
%     \textbf{Online model selection on IMDB (top row) and XSum-LLM (bottom row).}
%     (a, b) IMDB sentiment analysis with $T=50000$.
%     (c, d) LLM fine-tuning on XSum summarization with $T=1000$.
%     The right-side shared legend indicates the algorithms used in the cumulative-regret plots, while the right-side legends of the left-column plots indicate model configurations.
%     Shaded regions denote 95\% confidence intervals.
%     }
%     \label{fig:realworld_combined}
% \end{figure}


==> figure/tex/IMDB_regret.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[c]{0.75\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/images/IMDB_regret.pdf}
    \end{minipage}%
    \hfill 
    \begin{minipage}[c]{0.24\linewidth}
    \vspace{-0.5cm}
        \centering
        \includegraphics[width=\linewidth]{figure/images/legend_IMDB.pdf}
    \end{minipage}
    \vspace{-0.2cm}

    \caption{\textbf{Cumulative Regret on IMDB Dataset.} Performance comparison of CURE-UCB against baselines over a horizon of $T$=50,000, based on the reward functions depicted in Figure~\ref{fig:imdb_reward_only}. Shaded regions denote 95\% confidence intervals.
    \todo{Change size}}
    \label{fig:imdb_regret_only}
    \vspace{-0.3cm}
\end{figure}

==> figure/tex/IMDB_reward.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[c]{0.72\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/images/IMDB_reward.pdf}
    \end{minipage}%
    \hfill 
    \begin{minipage}[c]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/images/legend_IMDB_model.pdf}
    \end{minipage}

    \caption{\textbf{Reward Dynamics in Online Model Selection (IMDB).} Each line represents the validation accuracy of a distinct learning model configuration over time ($T$=50,000). Unlike synthetic settings, these real-world learning curves exhibit significant volatility and do not strictly adhere to smooth concave growth, presenting a challenging environment for horizon-dependent optimization.
     \todo{Change size}}
    \label{fig:imdb_reward_only}
    \vspace{-0.3cm}
\end{figure}

==> figure/tex/algo_desc.tex <==
\begin{figure}[t]
    \centering
    \tikzset{
        axis line/.style={->, thick, >=Stealth},
        history curve/.style={ultra thick, black}, 
        future curve/.style={thick, gray!50},      
        estimate line/.style={ultra thick, dashed, black}, 
        guide line/.style={ultra thick, dashed, green!50!black},
        guide line2/.style={ultra thick, dashed, r-ed},
        label text/.style={font=\tiny}
    }
    \def\RewardFunc(#1){0.6 * pow(#1, 0.45)}
    \definecolor{r-ed}{HTML}{1F77B4}
    \def\SlopeEarly{0.175} 
    \def\SlopeLate{0.125}

    \def\YMax{3.0}

    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
            \begin{tikzpicture}
                \def\Nc{2.0}        
                \def\End{8.0}       
                \def\TauTarget{3.0} 
                \def\CureTarget{5.0}
                
                \draw[axis line] (0,0) -- (9, 0) node[below, font=\normalsize] {$n$};
                \draw[axis line] (0,0) -- (0, \YMax) node[left, font=\normalsize] {$\mu_i(n)$};

                \draw[history curve] plot[domain=0:\Nc, samples=50] (\x, {\RewardFunc(\x)});
                \draw[future curve]  plot[domain=\Nc:9.0, samples=50] (\x, {\RewardFunc(\x)});
                
                \coordinate (Current) at (\Nc, {\RewardFunc(\Nc)});
                \coordinate (HorizonEst) at (\End, {\RewardFunc(\Nc) + \SlopeEarly*(\End-\Nc)}); 
                \coordinate (EstEnd) at (9.0, {\RewardFunc(\Nc) + \SlopeEarly*(9.0-\Nc)}); 
                
                \fill[pattern=north east lines, pattern color=green!50!black!30] 
                    (\Nc, 0) -- (Current) -- (HorizonEst) -- (\End, 0) -- cycle;
                % \draw[green!50!black, thick] (\Nc, 0) -- (Current) -- (HorizonEst) -- (\End, 0);
                \draw[green!50!black!50, thick] (\Nc, 0) -- (Current);
                
                \draw[red, ultra thick] (\End, 2.3) -- (\End,0);
                \node[above, red, font=\sffamily\small\bfseries, align=center] at (\End, 2.4) {Horizon\\Limit};
                
                \draw[orange, ultra thick] (\Nc, 2.3) -- (\Nc,0);
                \node[above, orange, font=\sffamily\small\bfseries, align=center] at (\Nc, 2.4) {Current\\Pulls};
                
                \draw[estimate line] (Current) -- (EstEnd);
                
                \coordinate (CUREPt) at (\CureTarget, {\RewardFunc(\Nc) + \SlopeEarly * (\CureTarget-\Nc)});

                \draw[guide line] (\CureTarget, 0) -- (CUREPt);
                \fill[green!50!black] (CUREPt) circle (2.5pt);
                \draw[->, green!50!black, thick] (CUREPt) -- ++(0, 0.8) node[above, font=\sffamily\small\bfseries] {CURE-UCB};
                
                
                
                \coordinate (TauPt) at (\TauTarget, {\RewardFunc(\Nc) + \SlopeEarly*(\TauTarget-\Nc)});
                
                \draw[guide line2] (\TauTarget, 0) -- (TauPt);
                \fill[r-ed] (TauPt) circle (2.5pt);
                \draw[->, r-ed, thick] (TauPt) -- ++(0.0, 0.5) node[above, font=\sffamily\small\bfseries] {\;\;\;\;R-ed-UCB};

                \node[below, label text,  font=\normalsize] at (\Nc, -0.18) {$N_{i,t\!-\!1}$};
                % \node[below, label text, rotate=-30, anchor=north west, font=\normalsize] at (\End, 0) {$N_{i,t\!-\!1}\!+\!(T\!-\!t)$};
                \node[green!50!black, below, label text, font=\normalsize] at (\CureTarget+0.3, 0) {$N_{i,t\!-\!1}\!+\!\frac{(T\!-\!t)}{2}$};
                \node[r-ed, below, label text,font=\normalsize] at (\TauTarget-0.1, -0.18) {$t$};

                % \draw[decorate, decoration={calligraphic brace, amplitude=4pt, mirror}, green!50!black, thick]
                %     (\Nc, -0.8) -- (\End, -0.8) node[midway, below=4pt, label text] {Remaining $T-t$};

            \end{tikzpicture}
        }
        \caption{Early Stage}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
            \begin{tikzpicture}
                \def\Nc{4.0}       
                \def\End{6.0}     
                \def\TauTarget{8.0} 
                \def\CureTarget{5.0}
                
                \draw[axis line] (0,0) -- (9, 0) node[below, font=\normalsize] {$n$};
                \draw[axis line] (0,0) -- (0, \YMax) node[left, font=\normalsize] {$\mu_i(n)$};

                \draw[history curve] plot[domain=0:\Nc, samples=50] (\x, {\RewardFunc(\x)});
                \draw[future curve]  plot[domain=\Nc:9.0, samples=50] (\x, {\RewardFunc(\x)});

                \coordinate (Current) at (\Nc, {\RewardFunc(\Nc)});
                
                \coordinate (EstEnd) at (9.0, {\RewardFunc(4.0) + \SlopeLate*(9.0-\Nc)});
                \coordinate (HorizonEst) at (\End, {\RewardFunc(\Nc) + \SlopeLate*(\End-\Nc)});
                
                
                \fill[pattern=north east lines, pattern color=green!50!black!30] 
                    (\Nc, 0) -- (Current) -- (HorizonEst) -- (\End, 0) -- cycle;
                % \draw[green!50!black, thick] (\Nc, 0) -- (Current) -- (HorizonEst) -- (\End, 0);
                \draw[green!50!black!50, thick] (\Nc, 0) -- (Current);
                \draw[red, ultra thick] (\End, 2.3) -- (\End,0);
                \node[above, red, font=\sffamily\small\bfseries, align=center] at (\End, 2.4) {Horizon\\Limit};
                \draw[estimate line] (Current) -- (EstEnd);
                
                \coordinate (CUREPt) at (\CureTarget, {\RewardFunc(\Nc) + \SlopeLate * (\CureTarget-\Nc)});

                \draw[guide line] (\CureTarget, 0) -- (CUREPt);
                \fill[green!50!black] (CUREPt) circle (2.5pt);
                \draw[->, green!50!black, thick] (CUREPt) -- ++(0, 0.5) node[above, font=\sffamily\small\bfseries] {CURE-UCB };

                \draw[orange, ultra thick] (\Nc, 2.3) -- (\Nc,0);
                \node[above, orange, font=\sffamily\small\bfseries, align=center] at (\Nc, 2.4) {Current\\Pulls};
                \coordinate (TauPt) at (\TauTarget, {\RewardFunc(\Nc) + \SlopeLate*(\TauTarget-\Nc)});
                
                \draw[guide line2] (\TauTarget, 0) -- (TauPt);
                \fill[r-ed] (TauPt) circle (2.5pt);
                \draw[->, r-ed, thick] (TauPt) -- ++(0, 0.5) node[above, font=\sffamily\small\bfseries] {R-ed-UCB};

                \node[below, label text, font=\normalsize] at (\Nc-0.45, -0.18) {$N_{i,t\!-\!1}$};
                % \node[below, label text, rotate=-30, anchor=north west, font=\normalsize] at (\End, 0) {$N_{i,t\!-\!1}\!+\!(T\!-\!t)$};
                \node[green!50!black, below, label text, font=\normalsize] at (\CureTarget+0.65, 0) {$N_{i,t\!-\!1}\!+\!\frac{(T\!-\!t)}{2}$};
                \node[r-ed, below, label text, font=\normalsize] at (\TauTarget, -0.18) {$t$};
                

                % \draw[decorate, decoration={calligraphic brace, amplitude=4pt, mirror}, green!50!black, thick]
                %     (\Nc, -0.8) -- (\End, -0.8) node[midway, below=4pt, label text] {Remaining $T-t$};

            \end{tikzpicture}
        }
        \caption{Late Stage}
        \vspace{-0.2cm}
    \end{subfigure}
    \caption{\textbf{Comparison of estimation behaviors: horizon-aware (\textcolor{green!50!black}{CURE-UCB}) vs. horizon-agnostic (\textcolor[HTML]{1F77B4}{R-ed-UCB}).} 
    The \textcolor{red!80}{Horizon Limit} denotes the maximum reachable point given the remaining trials.
    Since this horizon ($T-t$) is identical for all arms, we visualize CURE-UCB using its midpoint derived from the cumulative area; normalizing by this common factor preserves the arm ranking.    
    (a) Early Stage: R-ed-UCB remains conservative due to small $t$, whereas CURE-UCB targets a point closer to the horizon limit, enabling aggressive exploration.
    (b) Late Stage: CURE-UCB shifts to exploitation within the limit, while R-ed-UCB overshoots into the impossible region.
    }
    \vspace{-0.5cm}
    \label{fig:algo_desc}
\end{figure}

==> figure/tex/intro2.tex <==
\begin{figure}[t]
    \centering

    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figure/images/selection_trajectory.pdf}
        \caption{Selection trajectory}
        \label{fig:imdb_reward}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figure/images/criteria.pdf}
        \caption{Decision criteria at different $t$}
        \label{fig:imdb_reward}
    \end{subfigure}

    \caption{
    \todo{Change Figure. How to convey the intuition our algorithm works well?}
    }
    \label{fig:trajectory}
\end{figure}

==> figure/tex/ltf_explain.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]
        {./figure/images/LTF_explain.pdf}
    \caption{
    \textbf{Linear-then-flat approximation of reward dynamics.}
    Increasing and converging reward dynamics (left) are approximated
    by a linear growth phase followed by a flat phase (right).
    }
    \label{fig:ltf_explain}
\end{figure}

==> figure/tex/ranking.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/images/ranking_temp.pdf}
    
    \caption{\textbf{Ranking.}}
    \label{fig:ranking}
\end{figure}

==> figure/tex/regret_100k.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figure/images/temp_regret.pdf}
    
    \includegraphics[width=0.9\linewidth]{figure/images/legend_all_algorithms.pdf}
    

    \caption{\textbf{Performance in Concave Setting.} Average cumulative regret over $T=100,000$ rounds.}
\end{figure}

==> figure/tex/result_ltf.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/images/legend_all_algorithms.pdf}
    % \vspace{-0.3cm}
    \vfill
    \begin{subfigure}[b]{0.38\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={7bp 10bp 8bp 3bp}, clip]{figure/images/regret_ltf.pdf}
        
        \caption{\small Cumulative Regret} 
        
        \label{fig:ltf_regret}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={5bp 40bp 5bp 5bp}, clip]{figure/images/ranking_ltf_10000.pdf}
        \caption{\small Average Rank ($T$=10,000)}
        \label{fig:ltf_rank_10k}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={5bp 40bp 5bp 5bp}, clip]{figure/images/ranking_ltf_50000.pdf}
        \caption{\small Average Rank ($T$=50,000)}
        \label{fig:ltf_rank_50k}
    \end{subfigure}
    

     \caption{\textbf{Performance Analysis in LTF Setting.}  (a) Cumulative regret as a function of the time horizon $T$. CURE-UCB consistently achieves the lowest regret across all horizons. (b, c) Average Rank at $T$=10,000 (short horizon) and $T$=50,000 (long horizon), respectively. Lower rank indicates better performance. CURE-UCB maintains the lowest rank in both horizons. Shaded regions and error bars denote 95\% confidence intervals.}
    \label{fig:ltf_all_results}
    \vspace{-0.3cm}
\end{figure*}

==> figure/tex/tradeoff.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{./figure/images/tradeoff.pdf}
    \vspace{-0.1cm}
    \includegraphics[width=0.75\linewidth]{./figure/images/tradeoff_legend.pdf}
    \vspace{-0.1cm}
    \caption{\textbf{Illustration of the Horizon-dependent optimality.}  The optimal policy is inherently dependent on the remaining horizon $T$. (a) With a short horizon ($T=100$), the Early Peaker (Arm A) is optimal as it maximizes immediate cumulative rewards. (b) With a long horizon ($T=1000$), the Late Bloomer (Arm B) becomes optimal, as the massive future gain (hatched area) outweighs the initial deficit. This demonstrates that horizon-unaware strategies may fail to identify the optimal arm by neglecting the remaining duration.}
    \vspace{-0.1cm}
    \label{figure:tradeoff}
\end{figure}

==> figure/tex/win_rate_friendly.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{./figure/images/win_rate_friendly.pdf}
    \caption{\textbf{Win rate for rising friendly setting}}
    \label{fig:win_rate}
\end{figure}

==> figure/tex/win_rate_ltf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{./figure/images/win_rate_ltf.pdf}
    \caption{\textbf{Win rate for LTF setting}}
    \label{fig:win_rate}
\end{figure}

==> table/comparison.tex <==
\begin{table}[!ht]
\centering
\caption{Comparison of horizon-aware rising bandit algorithms.}
\label{tab:horizon_aware_comparison}
\begin{tabular}{lccc}
\toprule
 & & \multicolumn{2}{c}{Theoretical Result} \\
\cmidrule(lr){3-4}
Paper & Reward Class & Regret bound & \makecell{Uniform \\ dominance (LTF)} \\
\midrule
\citet{heidari2016tight} & Concave & \makecell{Sublinear \\ (no explicit order)} & \xmark \\
\citet{amichay2025rising} & Linear & $\tilde{\Theta}(T^{4/5}K^{3/5})$ & \xmark \\
CURE-UCB (Ours) & Concave & $\tilde{O}(\max\{KT^{2/3},\, KT^{q}\Upsilon(T,q)\})$ & \cmark \\
\bottomrule
\end{tabular}
\end{table}
